MoVer: Motion Verification for Motion Graphics Animations

While large vision-language models can generate motion graphics animations from text prompts, they regularly fail to include all spatio-temporal properties described in the prompt. We introduce MoVer, a motion verification DSL based on first-order logic that can check spatio-temporal properties of a motion graphics animation. We identify a general set of such properties that people commonly use to describe animations (e.g., the direction and timing of motions, the relative positioning of objects, etc.). We implement these properties as predicates in MoVer and provide an execution engine that can apply a MoVer program to any input SVG-based motion graphics animation. We then demonstrate how MoVer can be used in an LLM-based synthesis and verification pipeline for iteratively refining motion graphics animations. Given a text prompt, our pipeline synthesizes a motion graphics animation and a corresponding MoVer program. Executing the verification program on the animation yields a report of the predicates that failed and the report can be automatically fed back to LLM to iteratively correct the animation. To evaluate our pipeline, we build a synthetic dataset of 5600 text prompts paired with ground truth MoVer verification programs. We find that while our LLM-based pipeline is able to automatically generate a correct motion graphics animation for 58.8% of the test prompts without any iteration, this number raises to 93.6% with up to 50 correction iterations. Our code and dataset are at https://mover-dsl.github.io.

==> Makefile <==
# make -f Makefile_pdflatex

R = main

pdf: $(R).pdf

$(R).bbl: $(R).bib
	pdflatex $(R)
	bibtex $(R)
	pdflatex $(R)

$(R).pdf: *.tex $(R).bbl
	pdflatex $(R)



notes:
	pdflatex "\def\MakeWithNotes{}\input{$(R)}"

wo:
	pdflatex "\def\MakeWithoutNotes{}\input{$(R)}"

clean:
	rm -f $(R).log $(R).aux $(R).bbl $(R).blg $(R).out



==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.10.  Bug fixes.  Documentation update.

Version 2.09.  Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> evaluation.tex <==
\section{Results}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/fig_verification.pdf}
    \caption{Given an input animation, executing a verification program in \dslname{} outputs result messages indicating which parts of the animation satisfy the constraint predicates and which part fail. \maneesh{Let's talk about all these results figures.}}
    \label{fig:verification}
\end{figure*}

\maneesh{Should probably move this example to Section 3.1}
%
Figure~\ref{fig:verificationExample} shows an example animation and a 
\dslname{} verification program that checks for various
spatio-temporal properties we would like it to
include.
%
The verification program can be manually coded, or it can be generated from a text prompt using
LLM-based program synthesis as will describe in Section~\ref{sec:llmsynth}.

\maneesh{Should probably move this example to Section 3.2}
%
Executing a \dslname{} verfication program on an motion graphics animation yields a report specifying
the which logic statements and predicate‰s the animation successfully passes and which it fails (Figure~\ref{fig:verificationExample}).
\maneesh{Figure~\ref{fig:verification} visualizes this report 
for an example animation.}



Figures~\ref{fig:teaser} and Figures~\ref{fig:verification} show
examples of motion graphics animations generated with out LLM-based
synthesis and verification pipeline. \maneesh{More examples can be
  found in the video and supplemental materials.} In both cases the input
natural language prompt describes a variety of spatio-temporal properties
the animation should include.
%
%We can represent the constraints expressed by the prompt with
%predicates available in \dslname{} and compose a verification program
%as a collection of logical statements (top right of
%Figure~\ref{fig:verification}).
\maneesh{Next two sentences are essentially repeats of things we have already said. Probably need to
  focs on specifics of our example here.}
%
The LLM generated verification program
encodes these desired properties as logical statements
composed of \dslname{} predicates.
%
The LLM generated motion graphics animation program produces a
sequence of SVG frames and executing the verification program on the
animation produces a verification report (true/false values for each
logical statement and its constituent predicates) as visualized in the
Figures.
%
\maneesh{Probably need to just explain the example(s) teaser and here (or just here) with more specifics. Just jumping in on the verification result doesn't provide enough context. Need to talk about the input prompt (which feels a bit convoluted so we should talk about that) and animation as well as the verification.}
%
For example, the verification result in Figure~\ref{fig:verification}
indicates that, although the letter Y did border with E on its left
side at frame 80, it did not stay at that position until the end of
its translation (frame 100) as specified in the prompt.  \maneesh{Not sure I follow this specific example.}


%Here we demonstrate how \dslname{} can be applied to verify if an
%animation produced by our LLM animation program synthesizer fulfills
%all requirements expressed in an input motion prompt
%(Figure~\ref{fig:verification}), and subsequently how an LLM
%synthesizer can use the verification result to iteratively improve the
%animation (Figure~\ref{fig:iteration}).

%% \paragraph{Verifying a generated animation} As shown in Figure~\ref{fig:verification},
%% the input motion prompt describes a series of motions performed by three letters.
%% We can represent the constraints expressed by the motion prompt with
%% predicates available in \dslname{} and compose a verification program
%% as a collection of logical statements (top right of
%% Figure~\ref{fig:verification}).  Executing the verification program
%% against the animation program generated by our LLM synthesizer
%% produces result messages that show the boolean values of each
%% statement as well as its constituent predicates.  As shown in
%% Figure~\ref{fig:verification}, the verification result indicates that,
%% although the letter Y did border with E on its left side at frame 80,
%% it did not stay at that position until the end of its translation
%% (frame 100).
%% % that the letter Y did not end at a position where it only touch and do not overlap with the letter E, as required by the motion prompt.
%% Further, the translation of the letter S takes place over the same period of time as the translation of the letter Y. 
%% Our verifier indicates that this fails the requirement that these two translations should happen sequentially.

%\paragraph{Iteratively improve the generated animation}
% mention the human user can also make corrections too?

Figure~\ref{fig:iteration} shows the next two iterations of our synthesis and
verification pipeline for the example in Figure~\ref{}. In this case
we automatically fed the verification error report back to the LLM
animation synthesizer. After the first iteration the synthesizer is
verifier reports that the letter Y now properly border the letter E after being
translated, but that their respective translations still did not happen
sequentially.
%
In a second iteration the LLM synthesizer fixes this problem and every
statement and predicate in the verification program evaluates to true
confirming that the final animation correctly matches the input
prompt. 
%
\maneesh{Lace in more specificity perhaps or talk about specifics of both the teaser and this example. Not sure.}

%Once we have the verification result against an animation, we can
%directly feed the result messages, along with the \dslname{} DSL
%documentation and the verification program, back into the LLM
%animation synthesizer to ask it for correction.  As the LLM
%synthesizer has access to all the previous animations it has generated
%and the verification results for each of them, we are in essence
%supplying the LLM synthesizer with negative in-context examples to
%help it make corrections in an iterative manner~\cite{CITE}.  As shown
%in Figure~\ref{fig:iteration},in the LLM synthesizer's first attempt
%to improve the animation, running the verification program indicates
%that the letter Y now properly border the letter E after being
%translated, but their respective translations still did not happen
%sequentially.  We run the feedback loop again, and, in the second
%attempt, the remaining problem of non-sequential translations was
%fixed.  As all logical statements have evaluated to true, we exit the
%feedback loop and output the final animation.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/fig_iteration.pdf}
    \caption{Using the output of a \dslname{} verification program, we automatically feed the verification result back into the LLM animation program synthesizer to iteratively refine the animation until all checks are passed. }
    \label{fig:iteration}
\end{figure*}


\section{Evaluation}

We evaluate our motion graphics synthesis and verification pipeline in
two ways.  (1) We first test the accuracy of our LLM-based
verification program synthesizer in generating \dslname{} code from
natural language descriptions of a motion graphics animation.  (2) We
then test how many iterations our fully automatic pipeline requires to
generate an animation that successfully passes the corresponding
verification program.

\vspace{0.5em}
\noindent
{\bf \em Test dataset.}
For these evaluations we require a test datatest consisting of natural
language prompts describing a motion graphics animation and the
corresponding ground truth motion verification program. 
%
Because no such dataset is readily available we have synthetically
built one using a template-based approach in combination with a
generative LLM (Appendix~\ref{} details our approach for constructing
this test dataset).
Our test dataset is divided into four categories
%of prompts can corresponding
%\dslname{} verification programs, 
based on the types of \dslname{}
predicates they exercise.

%We generate four categories of prompts, parameterized by the presence of types of predicates in our DSL.
%\jiaju{The category names are temporary.}
%We present the categories below, and more details about how we generate prompts can be found in Section~\ref{sec:prompt_generation}.
\begin{enumerate}[leftmargin=0.5cm]
    \item {\bf \em Single atomic motion.}  Each text prompt describes
      only one atomic motion with up to seven of its attributes
      (Table~\ref{tab:predicates}). (e.g. ``Expand the square
      upwards.'').
      %No reference to other objects or motions appears
      %in this category.
    
    \item {\bf \em Spatially relative motion.}  Each text prompt
      describes a single atomic motion that is relative to the spatial
      position of another object to exercise predicates from the 2D
      rectangle algebra
      (Figure~\ref{fig:allen_rectangle}). (e.g. ``Move the square next
      to the circle.'').

    
    \item {\bf \em Temporally relative motions.}  Each prompt describes at
      least two atomic motions with relative temporal sequencing relations to
      excercise predicates from the Allen temporal interval algebra
      (Figure~\ref{fig:allen_rectangle}). (e.g. ``Move the square,
      while scaling the circle'').

    
    \item {\bf \em  Spatio-temporally relative motions}: Each prompt
      includes multiple motions with relative temporal and spatial
      relationships (e.g. ``Move the square next to the circle, while
      scaling the circle'').
\end{enumerate}

\maneesh{Should say how many prompts all together and in each category}

%% We evaluate 1) the LLM-based program synthesizer's ability to parse a
%% natural language motion prompt into a \dslname{} verification program
%% and 2) the LLM-based motion graphics generation pipeline's ability to
%% output an animation that pass all checks in the \dslname{}
%% verification program from an input prompt.

%% \subsection{Motion prompt dataset}
%% We build a dataset consisting of motion prompts and their
%% corresponding ground truth \dslname{} motion verification
%% programs. \jiaju{should we explain why not ground truth animation?}
%% %
%% % \jiaju{TODO: dataset composition}
%% We generate motion prompts in four categories, parametrized by the presence of types of predicates in our DSL.
%% \jiaju{The category names are temporary.}
%% We present the categories below, and more details about how we generate prompts can be found in Section~\ref{sec:prompt_generation}.
%% \begin{enumerate}[leftmargin=0.5cm]
%%     \item \textit{Single atomic motions.}
%%     Each motion prompt within this category describes only one atomic motion with its seven attributes (Table~\ref{tab:predicates}).
%%     No reference to other objects or motions appears in this category of prompts.
    
%%     \item \textit{Object-relative motions.}
%%     Each prompt in this category describes a single atomic motion in reference to another object (e.g. ``Move the square next to the circle.''). 
%%     Each prompt involves concepts related to the Rectangle Algebra (Figure~\ref{fig:allen_rectangle})
    
%%     \item \textit{Motion-relative motions.}
%%     Each prompt of this category describes at least two atomic motions with temporal sequencing relations (e.g. ``Move the square, and then scale the circle'').
%%     Each prompt invokes concepts related to the Allen' Interval Algebra (Figure~\ref{fig:allen_rectangle}).
    
%%     \item \textit{Object-and-motion-relative motions}:
%%     Each prompt includes multiple motions with temporal relations and references to other objects in the scene (e.g. ``Move the square next to the circle, and then scale it'').
%% \end{enumerate}

\input{table_eval_parsing}

\vspace{0.5em}
\noindent {\bf \em Accuracy of LLM-based verification program synthesizer.}
Table~\ref{tab:eval_parsing} reports the success rate for the
LLM-based \dslname{} synthesizer across the prompts in our test dataset.
To compute this success rate we first compute the string difference between the
LLM synthesized program and the corresponding ground truth and count a success only
when there is a perfect string match.
%
This is a stringest test for success as the underlying semantics of
the two programs may match even without an exact string match. But we
leave a looser comparison (e.g. at the level of AST matching) to
future work.
%
Overall, we observe that our LLM-based synthesizer achieves a high
success rate across all four types of prompts.  \maneesh{Probably need
  something here about the categories and differences between them.}


To better understand the generalization capabilities of our LLM-based
synthesis approach we have implemented a semantic
parser\,\cite{kamath2018survey} for converting a text prompt into a
corresponding \dslname{} program using a classical, rule-based
approach. Appendix~\ref{sec:semanticParser} describes the parser in
detail. As shown in Table~\ref{tab:eval_parsing} although the semantic
parser is fairly successful across our test set at \maneesh{XX}, it is
not quite as successful as the LLM-based approach across the four
prompt categories.
%
Examining the unsuccesful examplares we find that the LLM tends to
... \maneesh{say something about its problems -- that it can fail
  unexpectedly}.
%
In contrast the semantic parser has trouble ... \maneesh{say something
  about its problems. brittle for certain classes of prompts.}
\maneesh{Would we be better off dropping the semantic parser
  compoletely from this paper?}


\input{table_eval_pipeline}

\vspace{0.5em}
\noindent {\bf \em Number of automatic iterations required.}
Table~\ref{tab:eval_pipeline} reports the number of iterations our
fully automatic pipeline (with LLM-generated verification programs)
\maneesh{maybe we should do this with ground truth -- or maybe with
  both?} requires to produce a motion graphics animation that
successfully passes the corresponding verification program.
\maneesh{put stoppping limit in caption of table.}
%
%For each prompt in the test dataset we iteratively feed back the
%verification error report until all the verification tests pass, or we
%have performed \maneesh{XX iterations}.
We observe that our pipeline performs well in the 
prompt categories that do not include spatially relative motions.
outputting the correct animation directly without needing correction for XX\% of the prompts. \maneesh{Is this the best way to report this?}
%
For test prompts in the spatially relative and spatio-temporally
relative categories, we observe a drop in first attempt success rate
and an increase in the number of timed-out attempts.  Oour pipeline on
average needed \maneesh{X} number of attempts before producing an
animation that passes all the checks.  Examining the multi-attempt and
timed-out cases, we find that ...  \jiaju{TODO: some reasons I have
  thought of so far: 1) relative positioning requires computing
  various magnitudes and determining the center of rotation/scaling,
  which the LLM is known to be struggling with (CITE). 2) there are
  some cases when a more direct feedback that offer some potential
  solutions might be helpful, as the verification results only provide
  true or false.}  Notes: \jiaju{TOOD: also, can report by motion
  types, as the LLM struggles more when the motion type is not
  translation} Notes:
% \jiaju{TODO: can also present some interesting cases where the LLM did the unexpected e.g. the example of using both rotation and translation while the prompt only said rotate}




%% \subsection{Evaluation results}
%% \subsubsection{LLM-based verification program synthesizer}
%% \input{table_eval_parsing}
%% To evaluate how well our LLM-based synthesizer can parse an input motion prompt into the correct \dslname{} program, we built a rule-based semantic parser as the baseline.
%% The detailed implementation of the semantic parser can be found at Section~\ref{sec:semantic_parser}.
%% % \jiaju{TODO: Report the success rate of both parsers across categories}
%% We run both the LLM-based parser and the semantic parser on all XXXX prompts in our dataset and report the success rate in Table~\ref{tab:eval_parsing}.
%% We measure the string difference between the output of a parser and the ground truth verification program and count a complete match as success and otherwise failure.
%% Overall, we observe that the LLM-based synthesizer achieve high success rate across all four types of prompts.
%% This is validated by the comparison against the rule-based parser, which achieves a decent performance of XX\% across the board.


%% \subsubsection{Motion graphics generation pipeline}
%% \input{table_eval_pipeline}
%% We run our LLM-based motion graphics generation pipeline on all prompts in our dataset.
%% As described in Section~\ref{sec:llmsynth}, once an animation has been generated, we feedback it back along with the verification result for correction if the animation did not pass all verification checks.
%% We repeat the loop until either the LLM-synthesizer produces a fully-correct animation or until it reaches the maximum number of tries ($n=XXX$).
%% \jiaju{TODO: say that we manually inspect the final output animations to ensure that they indeed fulfills the requirements of the input motion prompt?}
%% % \jiaju{TODO: Report the number of tries across categories}
%% We report the results in Table~\ref{tab:eval_pipeline}.
%% We observe that the generation pipeline performances well in the categories without relative spatial positioning between objects, outputting the correct animation directly without correct in XX\% of the prompts.
%% When it comes to prompts in the object-relative and object-motion categories, we observe a drop in first attempt success rate and an increase in the number of timed-out attempts.
%% The LLM synthesizer on average needed X number of attempts before producing an animation that passes all the checks.
%% Upon examining the multi-attempt and timed-out cases, we make several observations on why the LLM struggled.
%% \jiaju{TODO: some reasons I have thought of so far: 1) relative positioning requires computing various magnitudes and determining the center of rotation/scaling, which the LLM is known to be struggling with (CITE). 2) there are some cases when a more direct feedback that offer some potential solutions might be helpful, as the verification results only provide true or false.}
%% Notes:
%% \jiaju{TOOD: also, can report by motion types, as the LLM struggles more when the motion type is not translation}
%% Notes:
%% % \jiaju{TODO: can also present some interesting cases where the LLM did the unexpected e.g. the example of using both rotation and translation while the prompt only said rotate}


==> introduction.tex <==
\section{Introduction}
\label{sec:introduction}

\maneesh{We need to decide what the main contributions of this work are. I don't think they are really
  about motion graphics -- that happens to be the domain and is important, but far more important are the
  ideas of using semantic parsing to do program verification of LLM generated motion graphics code. We need
  to put together a title that reflects the contributions and focus the paper from the beginning on the main
  problem we are solving and our corresponding contributions.}

% \maneesh{I think we need to open the introduction by talking about
% the problem we are trying to solve -- converting natural language
% descriptions of animation into motion graphics animations. The first
% paragraph(s) should motivate why this is an important problem and
% very quickly say that researchers have developed strategies for
% doing this in other domains. I wouldn't mention KeyFramer and
% LogoMotion here as those are not the major pubs in this direction of
% work. Those can come in related work. End by explaining that we are
% following in this line of work using an LLM to convert from natural
% language to motion graphics programs.}  what is motion graphics
Motion graphics is a type of animation widely used in advertising,
user interfaces, and digital storytelling.
% current approaches, why bad
Recent text-to-animation generation approaches~\cite{gal2024breathing,
  luo2023videofusion, chen2024videocrafter2, wang2023modelscope} have
made it possible to generate animations in a frame-by-frame
representation from natural language descriptions.
% program approach good, 
However, editing these low-level sequences of pixels and frames can be
tedious and time consuming.  In contrast, prior
work~\cite{zhang2023motion} has demonstrated that representing motion
graphics animations as objects and motions offer many advantages, such
as meaningful abstractions closely aligned with human cognition and
flexible and precise control parameters.
\maneesh{Not sure what the main point of this paragraph is. I think it is far too focused on Motion Graphics and not enough on the problem we are really aiming to solve -- program verification.}

% in other domains, what other people have done
Existing techniques have explored synthesizing programs from natural
language prompts for other visual tasks;
SceneCraft~\cite{hu2025scenecraft} uses large language models (LLMs)
to create 3D scenes as Blender programs, while
VISPROG~\cite{gupta2023visprog} and
ViperGPT~\cite{surismenon2023vipergpt} prompt LLMs to generate
programs in domain specific languages (DSL) for visual question
answering tasks.  We adopt this line of work to use an LLM as a
synthesizer to produce motion graphics programs from natural language
descriptions.
\maneesh{We don't need to say what others have done in the intro. I think we need to fist say
what problem we are addressing -- namely verification of LLM generated code.}


% \maneesh{This paragraph is very important as it
%   is introducing the key issue we will be solving. We have given the
%   high-level problem in the paragraph 1 -- natural language to motion
%   graphics animation. This paragraph needs to set up the more specific
%   problem of verification of LLM generated animation
%   code. Hallucination is not the same as producing outputs that do not
%   match the user's intentions. In this paper we should focus on the
%   latter, not the former. We don't need to bring in the prior work
%   in this paragraph. Instead the key thing is to state the specific problem of verification and then directly go to saying what we do in this paper.}
%% our focus of problem
However, solely relying on LLMs to interpret user prompts may produce
outputs that deviate from the intended constraints specified by a user
in the input prompt~\cite{tseng2024keyframer, liu2024logomotion}.
This can result in programs that are syntactically executable but
semantically incorrect or misaligned with user expectations.  For
example, ``translate the circles to the canvas center'' contains a
post-state constraint on the translation motion for the circle
objects, but the animation program generated by the LLM may violate
that constraint (Figure~\ref{fig:teaser}).  To fix this problem, the
user would need to manually inspect the rendered animation and adjust
corresponding parameters in the program.
\maneesh{This paragraph is partly setting up the problem we are addressing, thought it is long and it doesn't
  need to be in contrast to what others have done. It also doesn't introduce the issue of verification. We need to talk about the problem more
  generally. This introduction is focusing too much on prior work. Also we should
  avoid the term ``misalignment''. This is a poorly defined term. }

\maneesh{I think we need one paragraph that introduces the specific
  problem that we are going to focus on (namely verification of LLM
  generated animation) rather than all the text that we have so
  far. Next paragraph can say what we do.}


% \maneesh{This paragraph needs to explain the key idea of how we do verification. Specifically it needs to explain how we use a semantic parser (and say what a semantic parser is) to convert the prompt into first order logic -- combined with the notions of semantics of time. These sentences are going to be very important as they will tell the reader the main ideas/contributions of our verification approach. Need to also say human can be in-the-loop for correction after the verification finds an error. Remove the relationship to prior work here. Intro only needs to reference the most important prior work.}
% \maneesh{Should plan a teaser and what might be included in that. Also how it will be referenced in the introduction.}
%% our work
In our work, we introduce a novel text-to-animation system that
improves LLM-based program synthesis with a program verification
pipeline.
%% synthesis
To generate motion graphics programs, we prompt an LLM with a static
SVG image, documentation of an animation API, and natural language
descriptions of motions.
%% verification DSL
For program verification, we propose a first-order logic (FOL)-based
DSL that uses Neo-Davidsonian event
semantics~\cite{davidson2001logical, parsons1990events} to represent
various motion constraints expressed in the input prompt with a set of
predicates, such as a motion's \texttt{direction} and \texttt{origin}.
% notions of timing
In motion graphics, temporal sequencing of motions is just as
important as how each individual motion is carried out, so we adopt
Allen's interval algebra~\shortcite{allen1983interval} to model the
temporal relationship constraints between any two motions, like
\texttt{precedes(m\_1, m\_2)}.
% give some reason and benefit and example
The modularity and composability of our FOL DSL allow us to model
constraints expressed in complex natural language descriptions of
motions in the form of verification programs by joining constraint
predicates with logical operators (Figure~\ref{fig:teaser})
\maneesh{This paragraph is nice. I think we will need to demonstrate the composability. Two things though. Depending on the first paragraph and title the reader should know that we will be use an LLM to generate the code. This is not a contribution and the sentence on it should be either eliminated or shortened if possible. More importantly, This paragraph doesn't talk about closing the loop and feeding back the verification results to the user for manual correction or to the LLM for LLM-based correction. That is also a critical piece of this system.}

%% semantic parser
In order to produce these verification programs in a reliable,
deterministic manner, we build a rule-based semantic parser that
extracts motions constraints from natural language prompts, instead of
using another LLM~\cite{brown2024large}.
% we can handle conflated expressions
Unlike previous approaches, our parser uses dependency parsing and
fine-tuned text classification models to process prompts that contain
\textit{conflations}, a linguistic phenomenon in which a single
expression adds multiple constraints on a
motion~\cite{talmy1975motion}.  For example, ``expand'' is a single
verb that constraints both the motion \texttt{type} (scaling) and
\texttt{direction} (an increase in size).
%% human in the loop for correction
We execute the verification program against the rendered animation
produced by the animation program to check if all constraints are met
and inform the user with the verification results.  In case of
violations, the user can feed the results back into the LLM for
correction, improving program synthesis results in a human-in-the-loop
manner.
\maneesh{We can decide later if we need the detail on how the verifier work (first two sentences). We don't need to contrast with previous approaches.}

% \maneesh{Needs to end with sentences summarizing the results of our evaluation.}
%% evaluation
To evaluate our work, we first parameterized the space of natural
language descriptions of motions based on Talmy's framework of motion
semantics that categorizes motion into components such as Figure,
Manner, Path, and Ground~\cite{talmy1975motion}.  By generating
prompts across different dimensions of this taxonomy, we assess our
system's ability to produce accurate verification and animation
programs.  We also explore the effectiveness of various LLMs for
program synthesis and evaluate the impact of replacing components of
our deterministic verifier with LLMs.  \jiaju{summarize evaluation
  results} Finally, we demonstrate the expressiveness of our system by
showing a variety of result animations.  \maneesh{We probably need to
  emphasize the evaluation as being a bigger contribution. I don't
  think people have developed good methods for evaluating these tools
  and we should promise release of the test prompts and other things
  (e.g. gold parses, etc.). Should give numbers here about how well we
  perform on these tests and talk about the high-level vs. low-level
  parameterization of the prompts and prompt templates. }

\vspace{0.5em}
\noindent
In summary, we make two main contributions:
\begin{enumerate}
    \item A text-to-animation system that improves LLM-based program
      synthesis with a program verification pipeline that uses a
      semantic parser to convert natural language into verification
      programs with composable FOL-based motion and timing predicates.\maneesh{This should focus on semantic parsing-based verification using FOL and Allen stuff, not on text-to-animation system. Could have a second bullet point automatically looping that back to the LLM -- though we would want to fully automate this loop and check that it either converges or ends with an incorrect program -- we need to do this check anyway.}
    % \maneesh{Should emphasize further the approach to verification with semantic parsing and FOL and notions of timing.}
    \item A taxonomy of natural language prompts describing motions. We use this to show which types of prompts are challenging to LLMs but can be properly processed with our verification pipeline. \maneesh{Need to be more precise about this and its use in the context of evaluating the space of prompts in which our system can work over.}
    % \maneesh{Should better explain why this is important.}
\end{enumerate}


%% ------ introduction v 1.0 ------

%% motivate programs, turn focus to motion graphics
% Programs have been applied in many areas of computer graphics as
% structured, symbolic descriptions of complex visual tasks and
% contents, such as L-systems~\cite{guo2020lsystems} and fractals for
% procedural modeling and the GLSL language~\cite{rost2009glsl} to
% specify shaders.  In the domain of animation, Scalable Vector
% Graphics (SVG)~\cite{svg2} is a widely adopted representation of
% animated 2D vector graphics. Expressing animation as objects and
% motions offer many advantages over working directly with pixels and
% frames, such as meaningful abstractions closely aligned with human
% cognition and flexible and precise control parameters.

%% but writing them manually can be hard, so recent work on LLMs for program synthesis
% Despite these benefits of visual programs, authoring such programs
% manually can be challenging and time-consuming due to their inherent
% complexity and the need for domain expertise.
% %
% The emergence of large language models (LLMs) have enabled the
% possibilities of automatically synthesizing visual programs from
% textual prompts.
% %
% Recent work like VISPROG~\cite{gupta2023visprog} and
% ViperGPT~\cite{surismenon2023vipergpt} prompt LLMs with domain
% specific language (DSL) documentation to generate interpretable
% programs for visual question answering tasks.  Systems like
% KeyFramer~\cite{tseng2024keyframer} and
% LogoMotion~\cite{liu2024logomotion} leverage LLMs to translate natural
% language descriptions into SVG-based animation programs, simplifying
% the design process for motion graphics, a type of 2D animations used
% widely in advertising, animated logos, and digital storytelling.


% %% problem of recent work
% However, current LLM-based systems are susceptible to hallucinations,
% as they may produce outputs that deviate from the intended constraints
% specified by a user in the input prompt.
% This can result in programs that are syntactically executable but semantically incorrect or misaligned with user expectations.
% % prior verification work in image generation
% In the image generation domain, works like TIFA~\cite{hu2023tifa} and
% Davidsonian Scene Graph~\cite{cho2024davidsonian} uses LLMs to
% generate a list of requirements from an image prompt and uses a visual
% language model (VLM) to check if the generated images satisfy this
% list of requirements.


% %% our work
% Inspired by prior work, we introduce a novel text-to-animation system that improves LLM-based program synthesis with program verification.
% %% synthesis
% For program synthesis, we similarly leverage an LLM to generate animation code within a specified animation API. 
% %% verification
% For program verification, we propose a first-order logic (FOL)-based DSL that uses Neo-Davidsonian event semantics~\cite{davidson2001logical, parsons1990events} to represent various motion constraints expressed in the input prompt.
% In contrast to prior work that also uses LLM for verification~\cite{hu2025scenecraft}, we provide a rule-based deterministic semantic parser that converts natural language prompts into a verification program written in our FOL DSL.
% Executing the verification program checks if all constraints are met.
% If any violations are detected, they are automatically fed back into the conversation with the LLM for correction, improving program synthesis results.

%% evaluation
% Our evaluation includes developing a taxonomy of motion prompts based on Talmy's framework of motion semantics that categorizes motion into components such as Figure, Manner, Path, and Ground~\cite{talmy1975motion}.
% By generating prompts across different dimensions of this taxonomy, we assess our system's ability to produce accurate verification and animation programs. 
% We also explore the effectiveness of various LLMs for program synthesis and evaluate the impact of replacing components of our deterministic verifier with LLMs.

% %% summary of contributions
% \vspace{0.5em}
% \noindent
% In summary, we make two main contributions:
% \begin{enumerate}
%     \item A text-to-animation system that combines LLM-based program synthesis with FOL-based program verification.
%     \item A taxonomy of natural language prompts describing motion graphics.
% \end{enumerate}




% Program representations in computer graphics, such as L-system, shader, and SVG.
% producing these programs manually can be difficult, recent work explored synthesizing them with LLMs, such as VISPROG and VIPERGPT to visual qa, and KeyFramer and LogoMotion for text-to-animation.

% However,  because of LLM's hallucination problem, the result can be unpredictably wrong.
% a prompt may contain explicit constraints that the LLM violates.


% In our work, we propose a text-to-animation system wih program synthesis and program verification.
% We use a LLM to synthesis animation program written in a provided animation API
% In the program verification workflow, we parse prompt into a FOL-based verification program that reflects the constraints indicated by the prompt.
% executing the program returns results that show if all the constraints are satsified
% when violations are found, we automatically feed it into the conversation for LLM to fix it.

% To evaluate our work, we first propose a taxonomy of the prompt space.
% We base our taxonomy on Talmy's break down of motion semantics into Figure, Manner, Path, and Ground
% we generate prompts procedurally across different dimensions of the prompt space, and evaluate our system's ability generating correct programs given these prompts
% We evaluate our system with different LLMs for program synthesis, and also swap out differnet components of our deterministic verifier with LLMs.



% Contribution
% System
% Verifier, into program synthesis loop
% The way of performing verification for the animation prompts

% Evaluation
% Parametrized design space of inputs
% Why these are the relevant axes?
% Which part LLM works better? Which part for the verifier?
% Comparisons
% LLM parser
% Swap part of the rule-based parser pipeline


%         - contributions
%             - in the checks that we do and how we communicate the checks into the system
%             - writing checks and use the check results as feedback to the LLM to improve the program generation result
%                 - chooses what to check
%                     - what constraints can be generated from a prompt, and which of those are useful?
%                     - CONTRIBUTION: how much variability can the constraint identifier handle?
%                         - quantify what it can do and what can’t do
%                 - do the checking
%                     - evaluation: is the check api expressive enough?
%                         - “these functions cover large enough functionalities”
%                 - feedback to the program
%     - three parts!

% - evaluation
%     - pair input prompt with a bunch of programs
%         - some of which follows the prompt, some of which violates (parts of) the prompt
%             - EVALUATE: can the constraint finder identify the constraints
%             - EVALUATE: can these constraints be checked properly
%             - EVALUATE: are the constraint checking results helpful in correcting the violations in the original program?




% LocalWords:  GLSL shaders Scalable SVG LLMs VISPROG ViperGPT DSL
% LocalWords:  interpretable KeyFramer LogoMotion LLM TIFA SceneCraft
% LocalWords:  Davidsonian VLM Talmy's verifier allen modularity
% LocalWords:  composability parameterization composable


==> method.tex <==
\section{Method}

\maneesh{I don't follow the organization of this section. Perhaps we need to quickly walk through an overall pipeline figure (1 paragraph max). But the figure will have to be carefully designed. We should talk about that.}

\subsection{FOL-based Verification DSL}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figs/predicate_table.png}
    \caption{
        Our first-order logic DSL 
    }
    \label{fig:table_predicate}
\end{figure*}

Our verification programs are written in our verification DSL based on first-order logic (FOL).
The FOL-based DSL consists of functions and predicates (functions return boolean values) designed based on prior cognitive psychology literature that analyzes how people think about and describe objects and motions (see the full list in Table~\ref{fig:table_predicate}).
We can use these functions and predicates, along with logical operators, to build up logical statements that express complex descriptions of motions.
For example, we can express the natural language sentence ``translate the square upward by 100 px'' with $\exists \texttt{m. type(m, "translate")} \land \texttt{direction(m, [0, 1])} \land \texttt{magnitude(m, 100.0)} \land \texttt{agent(m, o)}$, where \texttt{o} is a variable representing the square.
%
% What are the entities (objects and motions)
% A single motion has a type, direction, etc
In our DSL, there are two basic variable types: objects that each has properties like shape, color, position, and size, and motions that each has attributes like type, direction, agent, etc (full list in Table~\ref{fig:table_predicate}).

% Describe the DSL (look at What’s Left)
% Given a set of motions and objects, can resolve the FOL predicates
Given an animation program, we resolve the logical statements and return verification results that describe which part of the animation fails the constraints expressed by the logical statements.
%
For an input animation program, we first convert it into a 2D array data representation that our DSL operates on.
Each row of the 2D array corresponds to an object in the animation program, and each column represents a frame.
For each cell $(i,j)$ of the 2D array, we store the transformation information applied to object $i$ at frame $j$.

\jiaju{TODO: describe in more detail, maybe per predicate}
Each predicate in our DSL then looks at every cell and checks if the content in that cell satisfy its input parameters.
If so, it marks that cell as true, and false otherwise.
As the result, each cell returns a 2D array of boolean values, and each logical operator, such as and and or, joins the results of different predicates by performing element-wise boolean operations.

% How you execute the predicate on the 2D table
% Give the table, describe each predicate


% \maneesh{Not sure what this subsection is for.}

% Object predicates:
% \begin{description}
%       \item[\texttt{shape(obj, shape\_str)}]
%       \item[\texttt{color(obj, color\_str)}]
% \end{description}

% \noindent
% Motion predicates:
% \begin{description}
%       \item[\texttt{type(mot, type\_str)}]
%       \item[\texttt{direction(mot, dir)}]
%       \item[\texttt{magnitude(mot, mag)}]
%       \item[\texttt{origin(mot, org)}]
%       \item[\texttt{duration(mot, dur)}]
%       \item[\texttt{agent(mot, obj)}]
%       \item[\texttt{post(mot, expr)}]
% \end{description}

% \noindent
% Interval predicates based on~\cite{allen1983interval}
% \begin{description}
%       \item[\texttt{preceds(motA, motB)}]
%       \item[\texttt{meets(motA, motB)}]
%       \item[\texttt{overlaps(motA, motB)}]
%       \item[\texttt{finished\_by(motA, motB)}]
%       \item[\texttt{contains(motA, motB)}]
%       \item[\texttt{starts(motA, motB)}]
%       \item[\texttt{preceded\_by(motA, motB)}]
%       \item[\texttt{met\_by(motA, motB)}]
%       \item[\texttt{overlapped\_by(motA, motB)}]
%       \item[\texttt{finishes(motA, motB)}]
%       \item[\texttt{during(motA, motB)}]
%       \item[\texttt{started\_by(motA, motB)}]
%       \item[\texttt{equals(motA, motB)}]
% \end{description}

\subsection{Semantic Parser}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figs/fig_parser.pdf}
    \caption{
        The processing pipeline of our semantic parser. 
    }
    \label{fig:parser}
\end{figure*}
    
% \maneesh{Will be a lot easier to understand with a concrete example of a prompt and figures illustrating the main ideas. It will be easier to update this section as well once figures have been added -- rough, even handdrawn is best for now. Opening should explain the overall goals and a high-level walkthrough of the steps of the approach and assumptions made at each step.}

% \maneesh{The current version of the methods section reads like a list of things we do and mostly suggests that we string together lots of previous tools. I think it will be much stronger if it is written to emphasize the key ideas that we are bringing to make everything work. For example why the six categories of motion attributes. How did we choose those? These like this should be emphasized at the very beginning of this section if possible.}

%% motion attributes
% \maneesh{Why these six categories?}
\jiaju{Might be better to talk about these motion attributes when
  introducing the FOL DSL}
By analyzing parameters in existing animation software and
API~\cite{TODO} and summarizing relevant prompts found in the
VidProm~\cite{wang2024vidprom} dataset, we identify seven types of
motion attributes onto which constraints can be placed: \textit{type}
(type of motion, one of translation, rotation, and scaling),
\textit{agent} (object that performs the motion), \textit{direction},
\textit{magnitude}, \textit{origin} (for rotation and scaling),
\textit{timing} (duration and sequencing), and \textit{post state}
(e.g. end at a specific position).
\maneesh{I don't follow why we are explaining what is in this paragraph. It seems out of place. Goal needs to be explained first. I also don't understand how these things are constraints. We do we mean by the term ``constraint''?}

The goal of our semantic parser is to extract these types of
constraints placed on motions and their sequencing from an input
natural language description of a motion graphics animation and to
assemble these constraints into a verification program in the
FOL-based DSL described above.
\maneesh{I don't follow this goal because I don't know what we mean by ``constraint'' and I don't understand how the DSL is FOL-based, or what it even means to be FOL-based.}
%
% \maneesh{Should motivate each part of the pipeline. An example prompt can help with this. In general each part/step/stage of the work should be motivated.}
%
As shown in Figure~\ref{fig:parser}, our semantic parsing pipeline
consists of four stages: (1) we resolve object and motion
co-references (e.g. identifying that ``it'' refers to ``the black
square'', (2) we break the input prompt into atomic sentences
without complex clauses such that each sentence describes one
continuous motion (e.g. breaking down ``it rotates, while expanding''
into ``it rotates'' and ``it expands'', (3) we build a list of
constraint predicates for information contained within each atomic
sentence (e.g. \texttt{type(m, ''rotate'')} and \texttt{magnitude(m,
  90)} from ``rotates by 90 degrees'', and (4) we compose the final
verification program by adding timing predicates that describe
inter-sentence sequencing relationships.
\maneesh{Instead of intra- and inter- sentence processing stages we should give those two stages more descriptive names. Stage 4 seems to be about sequencing and stage 3 about single motions, or some such.}

In contrast to prior approaches \maneesh{citations here}, our parser can extract multiple
constraints added by a single expression (conflation) with a
multi-label text classification model in Stage 3 (e.g. \texttt{type}
and \texttt{direction} from the verb ``expand'' in
Figure~\ref{fig:parser}).  We describe each stage of our pipeline in
detail below. \maneesh{This paragraph seems out of place. I don't follow what a conflation is from the previous discussion and because we haven't explained how our stages work I can't follow the differences with prior work. Needs to move elsewhere.}

\subsubsection{Stage 1: Object and motion co-reference resolution}
The goal of this stage is to identify segments of text that refer to
the same object or motion.
%so that we do not add duplicate predicates
%later in the pipeline.
%
To resolve co-references to objects, we use the fastcoref
model~\cite{otmazgin2022fastcoref}.  As shown in
Figure~\ref{fig:parser}, this places``The black square'' and
``it'' in the same co-reference cluster.
%
For motion co-reference resolution, we first identify event triggers
(words that introduce a motion) based a set of heuristics.
Specifically, for each noun and verb in the input prompt, we check if
its lemmatized form matches words that describe a motion in our
vocabulary (e.g. ``spin'' is a word that introduces a rotation
motion). \maneesh{What does ``in our vocabulary'' mean. Where does
  that vocabulary come from. Need to explain this in more detail
  because this sounds very brittle -- it sounds as if we are giving
  the system a pre-specified vocabulary.}  If there is a match, then
we mark it as an event trigger.  We then match event triggers to each
other by comparing their modifiers and their positions in a
sentence~\cite{ahmed2023lemmamatching, kenyondean2018lemmaheuristic}.
\maneesh{Need  more explanation of how this matching occurs. What is the algorithm. Can come after the example.}
For example, in the sentence ``The square spins. While rotating, it
also scales'', ``spins'' and ``rotating'' are identified as event
triggers.  Moreover, because they both operate on the same object, and
``rotating'' sits within a subordinate clause, then we identify them
as co-references referring to the same motion of rotation.
% \maneesh{We should motivate each step. Why do we need three different prior techniques to do the co-reference resolution. Need to include detail about what the trigger words are. Paper needs to be re-implementable after reading. Right now the text is a bit too vague for that.}

\subsubsection{Stage 2: Text simplification}
At this stage, we aim to break down the original input prompt into
atomic sentences that each describes a single continuous motion.
This stage sets up the extractions of intra- and inter-sentence
constraints later. \maneesh{The motivation sentence is not that useful. Should be motivated more in terms why it is necessary to do the simplification. The current motivation begs the question of why intra- and inter- sentence stages are necessary.}

%
Prior works on text
simplification~\cite{zhang2019generating, ferres2016yats} have identified six types of syntactic structures for
simplification: passive constructions, appositive phrases, relative
clauses, coordinated clauses, correlated clauses, and adverbial
clauses. \maneesh{Simplification in what sense? Should explain why these six structures are relevant to breaking the prompt into simple sentences -- e.g. sentences that describe a single motion.}
%
We do not simplify appositive phrases as they modify nouns and do
not often introduce new motions.
\maneesh{I don't understand the previous sentence because I don't know what an ``appositive phrase is''. Also why should I as a reader believe you that they do not introduce new motions.}
We also do not process correlated
clauses (e.g. either...or...) as they are rare when describing
motions.  \maneesh{Again, why should I believe you?} For passive constructions, we process them directly in the
next stage. \maneesh{Why are are forcing passive constructions into the next stage? If the passive construction includes multiple motions it should be handled here -- no? Otherwise I'm not sure what simplification is about breaking sentences into single motions.}

Therefore, we simplify three syntactic constructions at this stage:
\textit{Coordinated Clauses}, \textit{Adverbial Clauses}, and
\text{Relative Clauses}.  We first identify if any of these
constructions exists in the input prompt based on dependency relations
obtained with a roberta-based transformer
model~\cite{liu2019roberta, honnibal2020spacy} and then recursively perform the
following set simplification operations based on clause type, until no
more complex structures are present.

\paragraph{Coordinate clauses} We identify this type of clause by the presence of the conjunctive ``and''. 
We split the sentence based on the number of conjuncts and copy relevant sentence parts. For example, given ``Rotate the blue and black square.'', we would edit it to become ``Rotate the blue square'' and ``Rotate the black square.''

\paragraph{Adverbial Clauses}
This type of clauses usually joins two motions together, such as the
second sentence in Figure~\ref{fig:parser}.  We identify this
construction if a verb has the ``advcl'' dependency tag and a ``mark''
word (such as ``while'' and ''before'') is present. \maneesh{Where are the dependency tags coming from? What do they mean?}
%
We first check if the motion contained in the adverbial clause (``while expanding by 2'' in Figure~\ref{fig:parser}) is a co-reference or not.  \maneesh{How is the check done?}
If not, then we split the adverbial clause into a standalone sentence from the main clause as it introduces a new motion (sentences with yellow and blue underlines in Figure~\ref{fig:parser}).
Otherwise, we leave it as-is since it is adding a timing constraint to the motion described in the main clause.

\paragraph{Relative Clauses}
This construction is less common but we process it similarly as
adverbial clauses.  We identify this type of clauses by the presence
of a noun labeled as ``relcl.''
\maneesh{I don't understand this description. Where are the dependency labels coming from and what do they mean.}
We similarly check if the motion
contained in the relative clause is a co-reference or not, and only
split the sentence if it is not. 


\subsubsection{Stage 3: Intra-sentence processing}
% \maneesh{What is a ``single motion''?} 
% \maneesh{Why is this assumption a safe assumption at this point? Should talk about these assumptions in opening of this section.}
% We assume that each input is an atomic sentence that describes and modifies a motion, and the motion is introduced by a verb (e.g. the black square rotates by 90 degrees).
At this stage, the original input prompts has been processed into
atomic sentences where each one introduces a single continuous motion
(Figure~\ref{fig:parser}).  The goal of intra-sentence processing is to extract
motion constraint predicates from each sentence, including from
\textit{conflated} expressions. \maneesh{Need to explain what a ``conflated expression'' is earlier and provide an example.}

For each sentence, we first use a roberta-based transformer model~\cite{liu2019roberta} \maneesh{what is a Roberta based transformer model. Should cite it} to
obtain its syntactic dependency tree via
spaCy~\cite{honnibal2020spacy}, whose root node is the motion verb
(see Stage 3 in Figure~\ref{fig:parser}).
The root node and each of
its subtrees can be seen as a modifier that adds constraints to a
motion (e.g. ``by 90 degrees'' and ``around its center'' attached to
``rotates'' in Figure~\ref{fig:parser}). 

For each subtree, we identify what types of motion attributes the phrase is adding constraints to by classifying it with a fine-tuned sentence transformer. \maneesh{prev sentence is awk.}
Specifically, we use SetFit~\cite{tunstall2022setfit} to fine-tune a sentence transformer on a multi-label vocabulary dataset of example attribute descriptions we curated manually. \maneesh{Where does the vocabulary come from. How brittle is this. Need more detail.}
% conflation!!
In this way, we can account for conflation cases where a single phrase
introduces more than one constraint by adding predicates for each
label. \maneesh{I don't understand the previous sentence as I don't follow how well SetFit does the classification or knows to treat words that expand into multiple constraints.} As shown in Figure~\ref{fig:parser}, the verb ``expanding'' is
parsed into two constraints: \texttt{type(m\_3, ``scale'')} and
\texttt{direction(m\_3, [1.0, 1.0])}.

% clausIE
% \maneesh{I;m a bit lost. Not sure where we introduced parse trees and root nodes. Should illustrate these things. More importantly should motivate why we are doing each step before we describe the step. Why do we need the finetuned SetFit transformer and how exactly do we finetune it.}
%
% describe object predicates
%

For each type of constraint that a phrase adds, we further process the content in the subtree to parse out arguments for the corresponding predicate.
For example, we identify ``by 90 degrees'' as adding a constraint on the \texttt{magnitude} attribute of the rotation motion.
Within the subtree of the phrase ``by 90 degrees'', we then look for a node with part of speech NUM (i.e. the node of the text ``90'') and use it to construct the predicate \texttt{magnitude(m\_2, 90)}.
\maneesh{What is the algorithm for this parsing procedure?}
\jiaju{Need to add more details on how we process direction/magnitude for scale}

% \maneesh{How do we know if a subtree falls in the categories. What is the algorithm for identifying the constraint. Examples need to be accompanied by a general algorithm.}
% \jiaju{TODO: write this in more detail}

\subsubsection{Stage 4: Inter-sentence processing}
An important part of describing motion graphics is the sequencing of
motions.  In the last stage of our parsing pipeline, we iterate
through every atomic sentence and look for expressions that add
sequencing constraints between motions.  We again use a fine-tuned
transformer model for classification.
\maneesh{For classification into what? What exactly do we do? What is the algorithm?}
As shown in
Figure~\ref{fig:parser}, the word ``then'' signals that the rotation
motion needs to happen after the translation motion, and ``while''
indicates that the scaling needs to take place at the same time as the
rotation.  We map each of these words to their corresponding timing
predicates as described in Allen's interval
algebra~\cite{allen1983interval}.
\maneesh{This interval algebra needs to be described in more detail and likely with a figure.}
The final output verification
program is shown at the bottom of Figure~\ref{fig:parser}.
% For example, if a sentence contains the word ``then'' as an adverb modifying the verb, we create a timing predicate that checks whether if the motion described in this sentence takes place after the previous sentence (e.g. \texttt{preceds(m\_1, m\_2)}).
% \jiaju{TODO: write this in more detail}

% LocalWords:  DSL str dir dur preceds motA motB fastcoref Intra NUM
% LocalWords:  spaCy subtree SetFit finetuned finetune TODO expr pre
% LocalWords:  VidProm intra lemmatized roberta advcl relcl subtrees
% LocalWords:  prev awk


==> method2.tex <==
\section{Method}
\label{sec:method}

Our method takes a text prompt as input and generates a corresponding
motion graphics animation program in 3 main steps
(Figure~\ref{fig:pipeline}).
%
(1) A Motion Program Synthesizer uses in-context LLM-based program
synthesis to generate an SVG motion program.
%that represents each foreground object as an SVG group {\tt <g>}
%containing it's appearance and a sequence of per-frame motion
%transforms.
(2) A Prompt Parser converts $t$ into a FOL-based verification program
using our motion verification DSL.  \maneesh{We a explore two
  approaches to parsing in this work, a rule-based semantic parser and
  an in-context, LLM-based parser.}
%
(3) A Motion Verifier then applies the verification program to the SVG motion program
to check that space-time concepts mentioned in the prompt appear in the motion program.
%
If verification fails our system can automatically send the error
feedback to the synthesizer to update the program thereby supporting
iterative updates.
%
In addition a human user can examine the verification output and either
manually fix the motion program, or filter the feedback sent to the
synthesizer. \maneesh{Last sentence may not be necessary here.}

\maneesh{Might be able to kill the roadmap paragraph below.}
We first describe the Motion Program Synthesizer (Section~\ref{sec:synthesizer}) as
it generates the low-level SVG representation of motion our pipeline
operates on. We then describe our motion verification DSL
(Section~\ref{sec:dsl}). Next we explain how our Motion Verifier applies a
verification program to an SVG motion program
(Section~\ref{sec:verifier}). Finally we describe our Prompt Parsers
(Section~\ref{sec:parsers}).



\subsection{Motion Program Synthesizer}
\label{sec:synthesizer}

Our motion program synthesizer, follows prior work on in-context
LLM-based program synthesis\,\cite{}. \maneesh{see TIFA paper for references in
  addition to ViperGPT and VISPROG}. We provide a system prompt that
includes documentation for an SVG-based animation API and examples of
text prompts paired with corresponding output programs in this API
(see Appendix XX for the system prompt).
%
%Following prior work we use in-context LLM-based program
%synthesis\,\cite{see TIFA paper for references in addition to ViperGPT
%  and VISPROG}, with a system prompt that includes documentation
%for an SVG-based animation API and examples of prompts paired with
%corresponding output programs (Appendix XX shows the prompt.}
  %
While the animation API can be any high-level representation of the
SVG objects and their motions (e.g. a sparse keyframe based API such
as \maneesh{GSAP} \maneesh{Could we demonstrate a physics based
  API?}), our verifier operates on a low-level SVG representation
where each foreground object is represented as an SVG {\tt <shape>} ,
{\tt <g>}, or {\tt <image>} node with per-frame motion transforms,
similar to that used by Zhang et al.\,\shortcite{}.
%
Therefore our synthesizer also converts the high-level motion program
into the corresponding, generic low-level SVG motion program by
executing the high-level version and keeping track of the per object
transforms.

\subsection{Motion Verification DSL}
\label{sec:dsl}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{figs/predicate_table.png}
%     \caption{
%         Our first-order logic motion verification DSL. \maneesh{Needs to be made in Latex and also made to take up less room vertically.}
%     }
%     \label{fig:table_predicate}
% \end{figure*}

We have developed a domain specific language for verifying that
certain concepts related to space and time appear in an SVG motion
program.
%The language consists of functions and predicates 
%(i.e., functions that return boolean values)
The concepts are expressed as first-order logic predicates (functions
that return boolean values)
%in our language and are based on prior
%work in cognitive psychology\,\cite{} that has analyzed how people
%think about and describe animations
over variables representing objects $o_i$ and their
motions $m_j$.
%
For example, the predicate {\tt above($o_i$,$o_j$)} returns true for
each frame of the animation where object $o_j$ is above
$o_i$. \maneesh{above(o1,o2) is not directly in the table -- should give
  it as an example of a spatial concept.}
%
The predicate {\tt direction($m_i$, [0,1])} returns true for each frame where
motion $m_i$ is along the direction vector $[0,1]$ (i.e. rightwards).
%
And the expression $ \exists \texttt{m. type(m, "translate")} \land
\texttt{direction(m, [0, 1])} \land \texttt{magnitude(m, 100.0)} \land
\texttt{agent(m, iota(o, color(o,''black'')} \land
\texttt{shape(o,''square''))}$ returns true for each frame where a
square shaped object is translating upwards.  \maneesh{Might need to
  use $\iota$ symbol instead of iota(). Also maybe move long
  expression into a figure or table or equation block.}
%
Table~\ref{fig:table_predicate} shows the elements (predicates,
functions, boolean operators) of our language.


The predicates in our DSL are based on prior work from cognitive
psychology and linguistics that has analyzed how people think about
and describe meaningful spatio-temporal relationships in
animation\,\cite{Talmy,Tversky}. 
%
This work has shown that linguistic descriptions of animation
schematize the information to emphasize only the most salient
space-time configurations often without providing precise metric
properties in a absolute frame of reference (e.g., the square is at
(100,40) etc.), but rather in a frame of reference relative to other
objects (e.g., the square is next to the circle).
%
We build on Allen's\,\shortcite{} temporal algebra which provides a
formal representation for working with relative temporal
intervals as well as Balbiani et al.'s\,\shortcite{} rectangle algebra which
extends Allen's algebra to represent relative 2D spatial relationships.
%
Figure~\ref{} shows the various spatio-temporal relationships these
algebras can represent and our DSL provides predicates that can check
for each of them.


\input{table_predicates}
\subsection{Jiaju's Version: Motion Verification DSL}
We have developed \dslname{}, a domain specific language for verifying that concepts related to space and time expressed in natural language descriptions of motions are properly executed in a motion graphics animation.
%
We express these concepts as first-order logic predicates (functions that return boolean values) over variables representing objects $o_i$ and their motions $m_i$ ( Table~\ref{tab:predicates}).
%
The predicates in \dslname{} are based on prior work from cognitive psychology and linguistics that has analyzed how people think about and describe salient spatio-temporal relationships in animations~\cite{allen1983interval, talmy1975motion, Tversky}. 
%% concept of single motion
We organize these predicates into logical statements that describe \textit{atomic motions}, entities that have the seven attributes listed in Table~\ref{tab:predicates}.
For example, the expression $ \exists \texttt{m. type(m, "translate")} \land \texttt{direction(m, [0, 1])} 
\land \texttt{agent(m, iota(o, color(o,''black'')} 
\land \texttt{shape(o,''square''))}$ returns true for each frame where a square shaped object is translating upwards.
% \maneesh{Might need to use $\iota$ symbol instead of iota(). Also maybe move long expression into a figure or table or equation block.}
% the predicate {\tt direction($m_i$, [1,0])} returns true for each frame where motion $m_i$ is along the direction vector $[1,0]$ (i.e. rightwards).
%

%% allen and rectangle
To express various \textit{temporal} relations between atomic motions and different \textit{spatial} relations between their objects, we build on Allen's~\shortcite{allen1983interval} temporal algebra, which provides a formal representation for working with relative temporal intervals (Figure~\ref{fig:allen}), and Balbiani et al.'s~\shortcite{} rectangle algebra, which extends Allen's algebra to represent relative spatial relationships in the 2D space.
%
Figure~\ref{fig:allen} and \ref{fig:spatial} show the various spatio-temporal relationships these algebras can represent, and our DSL provides predicates that can check for each of them.
\jiaju{need to be clear here that we have all the low-level predicates as well as high-level ones. The examples below are the high level ones.}
% example temporal
For example, \texttt{while(m$_i$, m$_j$)} checks for whether the two motions have any amount of overlap across time.
% example spatial
The spatial predicate {\tt above($o_i$,$o_j$)} returns true for each frame of the animation where object $o_i$ is above $o_j$. 
% \maneesh{above(o1,o2) is not directly in the table -- should give it as an example of a spatial concept.}

%
% Table~\ref{fig:table_predicate} shows the elements (predicates,
% functions, boolean operators) of our language.

%
\jiaju{I like this sentence, but I am not sure if it should be here. I wonder if this can be moved to intro.}
This work has shown that linguistic descriptions of animation schematize the information to emphasize only the most salient space-time configurations often, without the need to provide precise metric properties in a absolute frame of reference (e.g., the square is at (100,40)), but rather in a frame of reference relative to other objects (e.g., the square is next to the circle).
%


\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{figs/fig_allen.pdf}
  \caption{
      Illustration of the 13 relations in Allen's Interval Alegrab and mappings into 
      timing concepts in our DSL. 
  }
  \label{fig:allen}
\end{figure*}

\subsection{Verifying an SVG Motion Program}
\label{sec:verifier}

Our Motion Verifier is responsible for checking whether an SVG motion
program is consistent with a motion verification program written in our DSL.
%
%More specifically it executes the verification program on the SVG
%motion program and
%
It outputs the set of frames that evaluate to false with respect to
each logical expression in the verification program.
%
%Our Motion Verifier is responsible for executing a motion verification
%program on an SVG motion program.  It outputs the set of frames that
%evaluate to false with respect to each logical expression in the
%verification program.


To do this we first convert the SVG motion program into a 2D array
where each row represent an object and each column
represents a frame of the animation. In each cell $(i,j)$ of the array
we store a motion information for object $o_i$ at
frame $f_j$.
%
%% Specifically we store information about the motion type (translation,
%% rotation or scale), direction (``clockwise'' or ``counterclockwise''
%% for rotations, a normalized tangent vector for translations, and a 2D
%% vector of scalefactors (in $x$ and $y$) for scale), magnitude, and
%% center (of rotation or of scale).
%
Specifically for each object we obtain its per-frame transformation
matrix from the SVG motion program and factor it into motion parameters for
rotation (e.g. angle), translation (e.g. direction and magnitude),
etc. and store these in the corresponding cells of the array.
%
We separately store static information for each object such as its color,
shape, and bounding box (in object local coordinates).
%


With these data structure in place we implement our DSL as follows.
%
%{\tt exists(var, expr)}: we recursively execute {\tt expr} 
%
We execute each logical predicate in the verification program on each
cell of the 2D (object $\times$ frame) array and mark the
corresponding cell of an output boolean matrix as true if the
predicate is satisfied and false otherwise. Thus each predicate
produces a 2D boolean matrix of size $|O| \times |F|$.
%
For example, executing the predicate {\tt type(m,''rotation'')} sets
matrix cell $(i,j)$ as true if object $o_i$ has a non-zero rotation
angle in frame $f_j$. Similarly, executing the predicate {\tt
  shape(o,''square'')} sets the entire matrix row $(i,*)$ to true if
object $o_i$ is square shaped. 
%
A predicate expression (i.e., {\tt expr}) combines the results of
multiple predicates by applying logical boolean operators (e.g. and,
or, not) element-wise on the predicate matrices.
%
%and we can apply boolean operators (e.g. and, or, not) element-wise to
%each entry in the matrix to combine the results of different
%predicates.

While many predicates primarily involve looking up information in the
animation and object data structures, predicates that compare the
timing of two motions or the bounding boxes of two objects (from the
Allen or rectangle algebras) are more complex. These require
comparisons between the starting and ending frames of the motions or
between the relative positions of the bounding boxes of the objects
(Figure~\ref{}).




\maneesh{----------- OLD TEXT ---------}



\subsection{Semantic Parser}
\label{sec:parsers}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figs/fig_parser.pdf}
    \caption{
        The processing pipeline of our semantic parser. 
    }
    \label{fig:parser}
\end{figure*}
    
% \maneesh{Will be a lot easier to understand with a concrete example of a prompt and figures illustrating the main ideas. It will be easier to update this section as well once figures have been added -- rough, even handdrawn is best for now. Opening should explain the overall goals and a high-level walkthrough of the steps of the approach and assumptions made at each step.}

% \maneesh{The current version of the methods section reads like a list of things we do and mostly suggests that we string together lots of previous tools. I think it will be much stronger if it is written to emphasize the key ideas that we are bringing to make everything work. For example why the six categories of motion attributes. How did we choose those? These like this should be emphasized at the very beginning of this section if possible.}

%% motion attributes
% \maneesh{Why these six categories?}
\jiaju{Might be better to talk about these motion attributes when
  introducing the FOL DSL}
By analyzing parameters in existing animation software and
API~\cite{TODO} and summarizing relevant prompts found in the
VidProm~\cite{wang2024vidprom} dataset, we identify seven types of
motion attributes onto which constraints can be placed: \textit{type}
(type of motion, one of translation, rotation, and scaling),
\textit{agent} (object that performs the motion), \textit{direction},
\textit{magnitude}, \textit{origin} (for rotation and scaling),
\textit{timing} (duration and sequencing), and \textit{post state}
(e.g. end at a specific position).
\maneesh{I don't follow why we are explaining what is in this paragraph. It seems out of place. Goal needs to be explained first. I also don't understand how these things are constraints. We do we mean by the term ``constraint''?}

The goal of our semantic parser is to extract these types of
constraints placed on motions and their sequencing from an input
natural language description of a motion graphics animation and to
assemble these constraints into a verification program in the
FOL-based DSL described above.
\maneesh{I don't follow this goal because I don't know what we mean by ``constraint'' and I don't understand how the DSL is FOL-based, or what it even means to be FOL-based.}
%
% \maneesh{Should motivate each part of the pipeline. An example prompt can help with this. In general each part/step/stage of the work should be motivated.}
%
As shown in Figure~\ref{fig:parser}, our semantic parsing pipeline
consists of four stages: (1) we resolve object and motion
co-references (e.g. identifying that ``it'' refers to ``the black
square'', (2) we break the input prompt into atomic sentences
without complex clauses such that each sentence describes one
continuous motion (e.g. breaking down ``it rotates, while expanding''
into ``it rotates'' and ``it expands'', (3) we build a list of
constraint predicates for information contained within each atomic
sentence (e.g. \texttt{type(m, ''rotate'')} and \texttt{magnitude(m,
  90)} from ``rotates by 90 degrees'', and (4) we compose the final
verification program by adding timing predicates that describe
inter-sentence sequencing relationships.
\maneesh{Instead of intra- and inter- sentence processing stages we should give those two stages more descriptive names. Stage 4 seems to be about sequencing and stage 3 about single motions, or some such.}

In contrast to prior approaches \maneesh{citations here}, our parser can extract multiple
constraints added by a single expression (conflation) with a
multi-label text classification model in Stage 3 (e.g. \texttt{type}
and \texttt{direction} from the verb ``expand'' in
Figure~\ref{fig:parser}).  We describe each stage of our pipeline in
detail below. \maneesh{This paragraph seems out of place. I don't follow what a conflation is from the previous discussion and because we haven't explained how our stages work I can't follow the differences with prior work. Needs to move elsewhere.}

\subsubsection{Stage 1: Object and motion co-reference resolution}
The goal of this stage is to identify segments of text that refer to
the same object or motion.
%so that we do not add duplicate predicates
%later in the pipeline.
%
To resolve co-references to objects, we use the fastcoref
model~\cite{otmazgin2022fastcoref}.  As shown in
Figure~\ref{fig:parser}, this places``The black square'' and
``it'' in the same co-reference cluster.
%
For motion co-reference resolution, we first identify event triggers
(words that introduce a motion) based a set of heuristics.
Specifically, for each noun and verb in the input prompt, we check if
its lemmatized form matches words that describe a motion in our
vocabulary (e.g. ``spin'' is a word that introduces a rotation
motion). \maneesh{What does ``in our vocabulary'' mean. Where does
  that vocabulary come from. Need to explain this in more detail
  because this sounds very brittle -- it sounds as if we are giving
  the system a pre-specified vocabulary.}  If there is a match, then
we mark it as an event trigger.  We then match event triggers to each
other by comparing their modifiers and their positions in a
sentence~\cite{ahmed2023lemmamatching, kenyondean2018lemmaheuristic}.
\maneesh{Need  more explanation of how this matching occurs. What is the algorithm. Can come after the example.}
For example, in the sentence ``The square spins. While rotating, it
also scales'', ``spins'' and ``rotating'' are identified as event
triggers.  Moreover, because they both operate on the same object, and
``rotating'' sits within a subordinate clause, then we identify them
as co-references referring to the same motion of rotation.
% \maneesh{We should motivate each step. Why do we need three different prior techniques to do the co-reference resolution. Need to include detail about what the trigger words are. Paper needs to be re-implementable after reading. Right now the text is a bit too vague for that.}

\subsubsection{Stage 2: Text simplification}
At this stage, we aim to break down the original input prompt into
atomic sentences that each describes a single continuous motion.
This stage sets up the extractions of intra- and inter-sentence
constraints later. \maneesh{The motivation sentence is not that useful. Should be motivated more in terms why it is necessary to do the simplification. The current motivation begs the question of why intra- and inter- sentence stages are necessary.}

%
Prior works on text
simplification~\cite{zhang2019generating, ferres2016yats} have identified six types of syntactic structures for
simplification: passive constructions, appositive phrases, relative
clauses, coordinated clauses, correlated clauses, and adverbial
clauses. \maneesh{Simplification in what sense? Should explain why these six structures are relevant to breaking the prompt into simple sentences -- e.g. sentences that describe a single motion.}
%
We do not simplify appositive phrases as they modify nouns and do
not often introduce new motions.
\maneesh{I don't understand the previous sentence because I don't know what an ``appositive phrase is''. Also why should I as a reader believe you that they do not introduce new motions.}
We also do not process correlated
clauses (e.g. either...or...) as they are rare when describing
motions.  \maneesh{Again, why should I believe you?} For passive constructions, we process them directly in the
next stage. \maneesh{Why are are forcing passive constructions into the next stage? If the passive construction includes multiple motions it should be handled here -- no? Otherwise I'm not sure what simplification is about breaking sentences into single motions.}

Therefore, we simplify three syntactic constructions at this stage:
\textit{Coordinated Clauses}, \textit{Adverbial Clauses}, and
\text{Relative Clauses}.  We first identify if any of these
constructions exists in the input prompt based on dependency relations
obtained with a roberta-based transformer
model~\cite{liu2019roberta, honnibal2020spacy} and then recursively perform the
following set simplification operations based on clause type, until no
more complex structures are present.

\paragraph{Coordinate clauses} We identify this type of clause by the presence of the conjunctive ``and''. 
We split the sentence based on the number of conjuncts and copy relevant sentence parts. For example, given ``Rotate the blue and black square.'', we would edit it to become ``Rotate the blue square'' and ``Rotate the black square.''

\paragraph{Adverbial Clauses}
This type of clauses usually joins two motions together, such as the
second sentence in Figure~\ref{fig:parser}.  We identify this
construction if a verb has the ``advcl'' dependency tag and a ``mark''
word (such as ``while'' and ''before'') is present. \maneesh{Where are the dependency tags coming from? What do they mean?}
%
We first check if the motion contained in the adverbial clause (``while expanding by 2'' in Figure~\ref{fig:parser}) is a co-reference or not.  \maneesh{How is the check done?}
If not, then we split the adverbial clause into a standalone sentence from the main clause as it introduces a new motion (sentences with yellow and blue underlines in Figure~\ref{fig:parser}).
Otherwise, we leave it as-is since it is adding a timing constraint to the motion described in the main clause.

\paragraph{Relative Clauses}
This construction is less common but we process it similarly as
adverbial clauses.  We identify this type of clauses by the presence
of a noun labeled as ``relcl.''
\maneesh{I don't understand this description. Where are the dependency labels coming from and what do they mean.}
We similarly check if the motion
contained in the relative clause is a co-reference or not, and only
split the sentence if it is not. 


\subsubsection{Stage 3: Intra-sentence processing}
% \maneesh{What is a ``single motion''?} 
% \maneesh{Why is this assumption a safe assumption at this point? Should talk about these assumptions in opening of this section.}
% We assume that each input is an atomic sentence that describes and modifies a motion, and the motion is introduced by a verb (e.g. the black square rotates by 90 degrees).
At this stage, the original input prompts has been processed into
atomic sentences where each one introduces a single continuous motion
(Figure~\ref{fig:parser}).  The goal of intra-sentence processing is to extract
motion constraint predicates from each sentence, including from
\textit{conflated} expressions. \maneesh{Need to explain what a ``conflated expression'' is earlier and provide an example.}

For each sentence, we first use a roberta-based transformer model~\cite{liu2019roberta} \maneesh{what is a Roberta based transformer model. Should cite it} to
obtain its syntactic dependency tree via
spaCy~\cite{honnibal2020spacy}, whose root node is the motion verb
(see Stage 3 in Figure~\ref{fig:parser}).
The root node and each of
its subtrees can be seen as a modifier that adds constraints to a
motion (e.g. ``by 90 degrees'' and ``around its center'' attached to
``rotates'' in Figure~\ref{fig:parser}). 

For each subtree, we identify what types of motion attributes the phrase is adding constraints to by classifying it with a fine-tuned sentence transformer. \maneesh{prev sentence is awk.}
Specifically, we use SetFit~\cite{tunstall2022setfit} to fine-tune a sentence transformer on a multi-label vocabulary dataset of example attribute descriptions we curated manually. \maneesh{Where does the vocabulary come from. How brittle is this. Need more detail.}
% conflation!!
In this way, we can account for conflation cases where a single phrase
introduces more than one constraint by adding predicates for each
label. \maneesh{I don't understand the previous sentence as I don't follow how well SetFit does the classification or knows to treat words that expand into multiple constraints.} As shown in Figure~\ref{fig:parser}, the verb ``expanding'' is
parsed into two constraints: \texttt{type(m\_3, ``scale'')} and
\texttt{direction(m\_3, [1.0, 1.0])}.

% clausIE
% \maneesh{I;m a bit lost. Not sure where we introduced parse trees and root nodes. Should illustrate these things. More importantly should motivate why we are doing each step before we describe the step. Why do we need the finetuned SetFit transformer and how exactly do we finetune it.}
%
% describe object predicates
%

For each type of constraint that a phrase adds, we further process the content in the subtree to parse out arguments for the corresponding predicate.
For example, we identify ``by 90 degrees'' as adding a constraint on the \texttt{magnitude} attribute of the rotation motion.
Within the subtree of the phrase ``by 90 degrees'', we then look for a node with part of speech NUM (i.e. the node of the text ``90'') and use it to construct the predicate \texttt{magnitude(m\_2, 90)}.
\maneesh{What is the algorithm for this parsing procedure?}
\jiaju{Need to add more details on how we process direction/magnitude for scale}

% \maneesh{How do we know if a subtree falls in the categories. What is the algorithm for identifying the constraint. Examples need to be accompanied by a general algorithm.}
% \jiaju{TODO: write this in more detail}

\subsubsection{Stage 4: Inter-sentence processing}
An important part of describing motion graphics is the sequencing of
motions.  In the last stage of our parsing pipeline, we iterate
through every atomic sentence and look for expressions that add
sequencing constraints between motions.  We again use a fine-tuned
transformer model for classification.
\maneesh{For classification into what? What exactly do we do? What is the algorithm?}
As shown in
Figure~\ref{fig:parser}, the word ``then'' signals that the rotation
motion needs to happen after the translation motion, and ``while''
indicates that the scaling needs to take place at the same time as the
rotation.  We map each of these words to their corresponding timing
predicates as described in Allen's interval
algebra~\cite{allen1983interval}.
\maneesh{This interval algebra needs to be described in more detail and likely with a figure.}
The final output verification
program is shown at the bottom of Figure~\ref{fig:parser}.
% For example, if a sentence contains the word ``then'' as an adverb modifying the verb, we create a timing predicate that checks whether if the motion described in this sentence takes place after the previous sentence (e.g. \texttt{preceds(m\_1, m\_2)}).
% \jiaju{TODO: write this in more detail}

% LocalWords:  DSL str dir dur preceds motA motB fastcoref Intra NUM
% LocalWords:  spaCy subtree SetFit finetuned finetune TODO expr pre
% LocalWords:  VidProm intra lemmatized roberta advcl relcl subtrees
% LocalWords:  prev awk LLM SVG Verifier Parsers keyframe GSAP Zhang
% LocalWords:  verifier et al spatio Balbiani


==> parsers.tex <==
\section{Semantic Parser}

\subsection{Semantic Parsing Pipeline}
\label{sec:semantic_parser}
%% define single motion
The goal of our semantic parsing pipeline is to convert a natural language description of motions into a verification program written in our motion verification DSL.
%
The primary challenge is to map each part of a natural language sentence into corresponding predicates with appropriate parameters. 
%
As shown in Figure~\ref{fig:parser}, our semantic parsing pipeline consists of five stages: 
(1) we resolve object and motion co-references (e.g. identifying that ``it'' refers to ``the black square''),
(2) we break the input prompt into atomic sentences, each of which describes a single motion (e.g. breaking down ``it rotates, while expanding'' into ``it rotates'' and ``while [it] expanding''),
(3) we extract a set of predicates from information contained within each atomic sentence (e.g. \texttt{type(m, "rotate")} and \texttt{magnitude(m, 90)} from ``rotates by 90 degrees'',
(4) we add timing predicates that constraint the relative sequencing of motions by examining timing-related phrases, and
(5) we compose the final verification program by using logical operators to chain predicates together.
% \maneesh{Instead of intra- and inter- sentence processing stages we should give those two stages more descriptive names. Stage 4 seems to be about sequencing and stage 3 about single motions, or some such.}

%% dependendy parsing
Our pipeline works with natural language sentences in the format of their dependency parsing trees.
We use a roberta-based transformer
model~\cite{liu2019roberta} trained as a dependency parser~\cite{honnibal2020spacy} to convert a sentence into a tree rooted at its main verb.
Each node is a word and the edge between the node and its parent is decorated with the grammatical dependency relationship between them. 
Other linguistic information like a word’s part of speech and lemma is also stored with a node.
For example, ``the square translates'' will be converted into a tree rooted at the verb ``translate''.
The noun ``square`` becomes the child of ``translate'' with the dependency tag as \textit{nsubj}, the nominal subject of the verb.



\subsection{Semantic Parser}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figs/fig_parser.pdf}
    \caption{
        The processing pipeline of our semantic parser. 
    }
    \label{fig:parser}
\end{figure*}



\subsubsection{Stage 1: Resolve object and motion co-references}
The goal of this stage is to identify segments of text that refer to the same objects or motions, as it is common to refer to previously mentioned entities in natural language.
%
To resolve co-references to objects, we use the fastcoref model~\cite{otmazgin2022fastcoref}.
As shown in Figure~\ref{fig:parser}, this places ``the black square'' and ``it'' in the same co-reference cluster.
%
For motion co-references, we identify \textit{motion verbs}, defined as verbs that are synonyms of either ``translate'', ``rotate'', or ``scale,'' and compare the content of their subtrees that each acts as a modifier for one of the seven attributes of the motion entailed by that verb.
If the content of the subtrees describing the same attribute match, we mark these verbs as co-references of each other.
For example, for the prompt ``The black square spins. While the square is rotating, the circle scales up.'' we would categorize ``spins'' and ``is rotating'' as co-references as they share the same motion type (rotation) and the same subject (the black square).
Note that verbs referencing previous motions need to sit within a subordinate clause (e.g. ``is rotating'' is within a adverbial clause), as we assume verbs in main clauses always introduce new motions.
% matching algorithm
% NOTE: More specifically, we first find pairs of verbs that are synonyms of each other, where the first verb in a pair appears earlier in the prompt and is in a main clause, and the second verb appears later and is in a subordinate clause.

% Take Example Input 2, we are going to compare the dependency parse trees of “the black square spins” and “while the square is rotating”

\subsubsection{Stage 2: Split motion sentences into atomic ones}
Our motion verification DSL is designed to chain together predicates that put constraints on \textit{single motions} and their temporal relationships, where we define a \textit{single motion} to mean a motion entity consisting of the seven attributes listed in Table~\ref{fig:table_predicate}.
%
Our semantic parser builds on the assumption that people would use a motion verb to introduce a new motion. 
Because English has syntactic structures that allow multiple verbs to be in the same sentence (``rotates'' and ``expanding'' in Figure~\ref{fig:parser}), the goal of this stage is to split them into atomic sentences that each only contain one motion verb as the tree root.
%
% splitting
For a given dependency parse tree, we find all motion verb nodes.
If any two of these nodes are directly connected and neither node is a co-reference of another motion, then we remove the edge between them.
This might leave one of the verbs without an object, such as the verb ``expanding'' in Figure~\ref{fig:parser}.
In this case, we look for the closest node with the dependency tag \textit{nsubj} (nominal subject) or \textit{dobj} (direct object) in the original tree and attach it to the dangling verb (e.g. adding ``it'' to ``expanding'').

%% collapsing
The English language also allows the use of an auxiliary verb in addition to the main verb to introduce a motion, such as “animate the square to rotate” and “make the square expand”.
The dependency trees of these constructions will have these non-motion verbs (``animate'' and ``make'') as roots.
We resolve this by combining the pair of main and auxiliary verb into one node and reattaching their original subtrees to be under the combined node.

\subsubsection{Stage 3: Extract motion attribute predicates}
The goal of this stage is to extract information from each atomic sentence to output a set of predicates that put constraints on various attributes of a single motion described by that sentence.

%% root as type and child
We first classify the root verb node into one of ``translate'', ``rotate'', and ``scale'' to build the predicate \texttt{type(m, <type>)}.
Then, we find the verb node's direct subtree with a \textit{nsubj} or \textit{dobj} as the content of that subtree contains information about \texttt{agent()}.
Within that subtree, we look for words that describe the color and shape of that object and use those words as parameters for the \texttt{shape()} and \texttt{color()} predicates.
If a node within that subtree has a lemma of ``every'', ``each'', and ``all'', we mark this agent as plural and use \texttt{all()} later instead of \texttt{iota()}.

%% each subtree is a modifier
For the rest of the direct subtrees, we assume that each acts as modifiers that add additional constraints to the motion.
%% relative
We first search within those subtrees to look for mentions of other objects and build predicates for them with the same process described above.
These objects act as reference objects to be used as parameters for various predicates.
%%
In order to map the contents of direct subtrees to corresponding predicates in our DSL, we use SetFit~\cite{tunstall2022setfit} to fine-tune a sentence transformer on a multi-label vocabulary dataset of attribute descriptions we curated manually (e.g. mapping ``upwards'' to \texttt{direction()}).
%% conflation
The key reason behind a multi-label classifier is to handle the linguistic phenomenon of ``conflation'', where a single expression can contain multiple categories of constraints.
For example, our transformer-based classifier will map ``expanding'' in Figure~\ref{fig:parser} to both \texttt{type()} and \texttt{direction()}, as it signals an upward scaling motion.

%% subtree splitting
There are cases where different prepositional phrases are not directly being attached to the verb, although it is semantically modifying it.
In those cases, our transformer classifier will not be able to classify the subtree into any categories. 
To address this, we split it into smaller trees at each prepositional node, and resubmit each tree segment into the transformer for classification.
\jiaju{short example here?}

%% extract parameters
After a subtree is being mapped to corresponding predicates, we extract relevant parameters for the predicates as follows:
\jiaju{might want to shorten this}

% \vspace{-5mm}
% \begin{description}
\begin{description}[style=unboxed,leftmargin=0.5cm]
    \item[\texttt{direction()}]
    We use another fine-tuned sentence transformation to classify the subtree text into one or more of \{up, down, left, right, clockwise, counterclockwise, x-axis, y-axis\}.
    If the type of motion is translation, we map up to [0,1], down to [0, -1], left to [-1, 0], and right to [1, 0].
    If the type of motion is rotation, we map clockwise to ``clockwise'' and counterclockwise to ``counterclockwise''.
    If the type of motion is scaling, we map up to +1, down to -1, x-axis to [1,0], and y-axis to [0,1]. If no axis is specified, then we use [1,1]. We then output the final direction is up/down * axis. For example, ``up in x'' is [1, 0]
    
    \item[\texttt{magnitude()}]
    We look for node with the part of speech \textit{NUM} and use that as the parameter if the motion type is translate or rotate
    If the type is scale, we do NUM $\cdot$ axis with the axis vector obtained from before
    
    \item[\texttt{origin()}]
    We check if the subtree text contains a string pattern of (num1, num2) and use those as absolute parameters.
    If a reference object has been extracted from this subtree, we use that as the parameter instead.
    
    \item[\texttt{duration()}]
    We look for node with type “nummod” or parts of speech as NUM and use that as the parameter.
    
    \item[\texttt{post()}]
    We use a separate transformer classifier to convert the subtree text to its corresponding spatial concept predicate, with arguments being the current motion agent and the reference object.
\end{description}

\subsubsection{Stage 4: Add timing constraints}
The goal of this stage is to parse out words or phrases that add timing constraints between any two single motions.
For each atomic sentence’s dependency parse tree, we again use the fine-tuned sentence transformer to classify its subtrees that have not been process in the last stage. 
We only handle one label at this stage: timing
If a timing subtree is found, we use another transformer classifier to map the subtree text into one of the timing predicates in our verification DSL \jiaju{be more specific?}.
\jiaju{Add details about how parameters are determined}

\subsubsection{Stage 5: Write an motion verification program}
We output the final program by using \texttt{and} to join together predicates that belong to the same variables.
We use \texttt{exists} for a motion if it’s not involved in any timing predicates, and use \texttt{iota} otherwise.


==> prompt_space.tex <==
\section{Motion Prompt Taxonomy}
% parametrize
% evaluate the space that our approach will work over
% being able to directly use a prompt templates and generate prompt

\maneesh{Need to motivate the need for a prompt space taxonomy in a sentence or two here.}

We characterize the space of motion prompts by adopting Talmy's
theoretical framework that a motion event consists of fundamental
semantic elements like Figure, Ground, and
Path~\cite{talmy1975motion}. \maneesh{This needs to be expanded. I
  don't buy that these things are ``fundamental''. If we are going to
  claim that we need to provide more of an argument about why they are
  fundamental. Also need to define what these terms Figure, Ground,
  Path mean. The definitions below seem long. I think we need to figure out
  how to condense the definitions and really focus on how we produce the prompt
  templates and the algorithmic generation of prompts according to the templates. Also the low level
parameterization doesn't seem to appear here.}


\subsection{Figure}
Figure refers to the moving entity in a motion.
The entity can be an \textit{individual} object, such as ``the black square'', or a \textit{group} of objects, like ``all circles.''

When describing motions, we can refer to individual objects
(e.g. ``The black square moves to the right, and the blue square moves
to the left''), or we can specify them collectively (e.g. ``The
squares move closer to each other'')

\subsection{Ground (Reference Object)}
\jiaju{Frame of reference is NOT ground}
% Frame of reference
Ground refers to the frame of reference.  In linguistics, there are
three main types of frame of reference, which all have their
equivalence in computer graphics terms: \textit{intrinsic} (object
coordinate system), \textit{relative} (camera coordinate system), and
\textit{absolute} (world coordinate system). The relative type is a
ternary system that describes relationships in terms of the position
of an object, the viewpoint of the perceiver, and the position of
another object.  When viewing a motion graphics animation, we assume
that the viewer has a fixed point of view, so we do not consider the
relative type of frame of reference in our taxonomy.

\paragraph{World Coordinate System}
% world system
The world coordinate system (absolute) describes the relationship
between an object and a fixed frame of reference, which in our case is
the SVG coordinate system.  For example, ``translate the black square
to the right'' means to translate the black square object towards the
right side of the SVG scene.

\paragraph{Object Coordinate system}
% relative 
The object coordinate system (intrinsic) describes the relationship between an object and a referential object in the latter object's coordinate system.
For example, in the prompt ``move the black square to the top of the red circle,'' the top of the red circle might not align with the top of the SVG coordinate system (positive y-direction) as the circle could have been rotated.

\subsection{Path}
% how do you describe the path an object should take?
% different ways to describe the same motion
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/fig_path.pdf}
    \caption{Example scene to demonstrate various ways of specifying a path}
    \label{fig:path}
\end{figure}

Path refers to the course of a motion taken by the Figure.
Based on the seven types of motion attributes that we identified above, we can fully specify a path in the following ways:
\begin{itemize}
    \item Type + Direction + Magnitude + Origin
    
    ``The red circle rotates around the canvas center by 90 degrees clockwise.''
    
    \item Type + Post State + Origin
    
    ``The red circle rotates to coincide with the blue circle around the canvas center.''
\end{itemize}



% It can be categorized into two types based on telicity, which means whether a motion has a specific endpoint or not. There are two types of telicity: \textit{telic} and \textit{atelic}

% \paragraph{Telic}
% A telic motion has a specified endpoint for the motion to be considered completed. For example, ``scale the square up by 2'' is a telic motion as the scaling is considered finished when the square has doubled its size.
% In our space, a telic motion can be specified by describing the magnitude of a motion (e.g. ``rotate the triangle by 90 degrees'') or the post state of motion (e.g. ``shift the circle to the center of the SVG'').

% \paragraph{Atelic}
% An atelic motion does not have a specific endpoint. For example, ``rotate the triangle around the blue circle'' and ``translate the triangle upward'' are atelic because they can continue indefinitely.
% In our space, we can specify atelic motions by providing information on direction and origin, as shown in the examples above.

% source
% goal
% change of direction

% english is motion + manner
% path and ground through prepositional phrases

% path + ground
% he drove to home, to home is path (to home) + ground (home)

% serilizations
% compound verb
% satellite being packed into compound verb

% ground - frames
% intrinsic
% relative
% absolute

% path
% telicity
% granularity. Slobin (2004a)

% scalar change
% non-scalar change


% \subsection{Manner}
% \jiaju{TODO: need to flesh out the categories of Manner}

% Manner can have many subcategories. In our case, the relevant dimensions are: mode (type of motion) and timing (intrinsic speed of a motion and sequencing between motions).

% \paragraph{Mode}

% \paragraph{Timing}
% intrinsic timing
% sequencing

% speed

% compound action
% force exertion

% LocalWords:  Talmy's parameterization perceiver SVG


==> related_work.tex <==
\section{Related Work}
\label{sec:related}

\maneesh{12-31-24: Going to skip over this section for now except for note in FOL subsection. But we should think about where we might be able to shorten it.}

\subsection{Classic Text-to-Animation Systems}
% \maneesh{I would try to make this section shorter by writing sentences that can reference multiple papers together.}
% survey paper
Before the prevalence of LLMs, classic text-to-animation systems uses various natural language processing techniques to convert natural language descriptions into animations~\cite{bouali2023review}.
%
Early text-to-animation systems like CarSim~\cite{aakerberg2003carsim} use regular expressions to find verbs and classify them using WordNet.
It then maps categorized actions to animations.
%
Cardinal~\cite{marti2018cardinal} adds co-reference resolution and extracts triplets of subjects, actions, and objects and verb modifiers.
% It uses the Unity 3D engine for animation rendering.
%
Zhang et al.~\shortcite{zhang2019generating} extends Cardinal by adding a text simplification stage that breaks down complex clauses into simpler ones for downstream processing to support a wider variety of input language.
It also uses a semantic role labeler to extract key-value pairs of visual elements and actions, referred to as Action Representation Fields (ARF).

% \maneesh{Need to always close RW paragraphs by saying how we differ or why these approaches cannot solve the problem. Need to state their limitations.}
An important aspect that this line of work overlooks is the \textit{conflation} of expressions in motion descriptions (e.g. ``contract'' is a single word that describes a scaling motion with a decrease in size)~\cite{talmy1975motion}.
In our work, we fine-tune a sentence transformer to assign multiple classification labels to a phrase to properly process conflated expressions.
Moreover, we process input natural language prompts for the purpose of animation verification, instead of animation generation.


% \maneesh{I might have one subsection on text-to-animation without LLMs and one for work that uses gen AI for this. Are KeyFramer and LogoMotion the only two that use LLMs. I think we need to check more thoroughly. Also need to problem consider video generation and perhaps things like ToonCrafter. Will need to figure out how t organize these sections with respect to the Program Synthesis stuff.}
\subsection{Foundation Model-Based Text-to-Animation Systems}
%% text-to-video
A body of work has trained end-to-end models to generate animations conditioned on an input image and a text prompt.
ModelScope~\cite{wang2023modelscope} is a latent video diffusion model built on image diffusion models.
VideoCrafter~\cite{chen2024videocrafter2} focuses on preserving the structure and style of the input image.
Videofusion~\cite{luo2023videofusion} conditions the generation with captions extracted from the input image.
%% text-to-video as priors
Gal et al.~\shortcite{gal2024breathing} leveraged these text-to-video models as priors to animate input vector sketches conditioned on textual prompts.
% bad because of frame to frame representation
However, these methods do not have a mechanism for users to iteratively improve the generation results.
More importantly, all of these methods produce animations as a sequence of frames in pixels or vector vertices, making it difficult to edit the results~\cite{zhang2023motion}.

%% LLM
%% keyframer
On the other hand, some recent work leverages LLMs to produce animations as programs.
KeyFramer~\cite{tseng2024keyframer} prompts an LLM with SVG code and an animation description to generate an animation program written in CSS.
%% logoMotion
LogoMotion~\cite{liu2024logomotion} extends this work by using a vision language model (VLM) capable of processing SVGs as images.
%
Both works have reported that LLMs often produce results misaligned with the users' requirements.
% \maneesh{Seems like we will need to compare to these methods. Need to state their limitations.}
While KeyFramer did not address this limitation, LogoMotion adds a program repair process to help users debug wrongly generated programs, but their process is confined to only static comparisons between the target and last frames of a rendered animation.
%
% \maneesh{Why is our work better than the previous tools.}
In our work, we propose a FOL-based verification DSL consisting of motion and temporal relation predicates that can be composed to express complex constraints stated in the textual prompts.
We inform the user with the verification results, supporting them to fix issues in the program directly or feed them back to the LLM for automatic improvement.
% propose a deterministic semantic parsing pipeline to produce verification programs that represent constraints needed to be satisfied instead of directly outputting animations.


% \maneesh{May need to come before the section on Davidsonian graphs.}
\subsection{Semantic Parsing into First-order Logic Forms}
\maneesh{We probably need a background section explaining FOL in our context and Allen intervals in our context -- or perhaps they can be folded into the methods description. But some (or maybe all) of this text would then go there.}
Neo-Davidsonian event semantics~\cite{parsons1990events,
davidson2001logical} is a formalism that can express natural language descriptions of events in the form of first-order logic statements.
It treats events, such as motions, as a unary predicate, and additional modifiers (e.g., adverbs) can be added with conjunctions and disjunctions to allow for flexible representation of complex sentence structures.
For example, ``translate upward'' can be expressed as $\exists \texttt{e.} \texttt{translate(e)} \land \texttt{upward(e)}$.
%% weakly surpervised paper
Artzi and Zettlemoyer~\shortcite{artzi2013mapping} applied this formalism to interpret and execute natural language instructions for navigation.
They use a weighted linear CCG grammar to parse natural language into logical forms. 
%% programport
Wang et al.~\shortcite{wang2023programmatically} similarly uses a CCG parser to convert natural language instructions for a robotic arm into domain-specific manipulation programs.
%% google transforming paper
Reddy et al. proposed a dependency-parsing based approach for semantic parsing into Neo-Davidsonian logical forms~\cite{reddy2016transforming}.
After obtaining a dependency tree of an input sentence, they flatten the tree via binarization and convert the binarized tree into logical statements via a set of conversion rules.
%% what's left
More recently, Hsu et al.~\cite{hsu2024left} uses an LLM as a domain-independent semantic parser to produce logical forms of input natural language questions for visual reasoning.

% \maneesh{Why are subordinate clauses an issue? If this is important we should stress that we handle them.}
% \maneesh{Why are simple sentences a problem?}
However, inputs in these works are mostly simple sentences without complex subordinate clauses.
This means that they do not need to consider intra- and inter-sentence relationships that are prevalent and essential in the descriptions of motions, such as object co-references and motion sequencing.
%
In our work, we construct a semantic parser capable of handling complex inter-sentence relations like object and motion co-references and event sequencing expressed through various subordinate clauses.


\subsection{Program Synthesis and Verification}
% VisProg and ViperGPT
VISPROG~\cite{gupta2023visprog} and ViperGPT~\cite{surismenon2023vipergpt} are neuro-symbolic methods demonstrating the LLMs' abilities to generate programs for visual question answering tasks without the need of additional training.
Given a description of available functions in a DSL, corresponding usage examples, and a natural language prompt of the visual question, both of these works can generate a program that returns answers to the input question upon execution.
% \maneesh{We should talk about the limitations of these methods in more detail.}
However, in case of wrong results being produced by the programs, the user needs to manually inspect the programs for debugging.

% TIFA
Prior works in image generation have used LLMs and VLMs to verify if the generated outputs faithfully follow the input descriptions.
For a prompt like ``a person sitting on a horse in air over gate in grass with people and trees in background,'' TIFA~\cite{hu2023tifa} uses an LLM to generate question-answer pairs (e.g. [``Is the horse in air'', ``Yes'']).
It then uses a VLM to answer these questions about the generated images.
The more questions are correctly answered, the higher the faithfulness is for that image. 
%%VP T2I
VPEval~\cite{cho2023vpt2i} uses an LLM to generate visual programs to evaluate text-to-image generation results.
% Davidsonian
Cho et al.~\shortcite{cho2024davidsonian} expanded on this approach by using a davisonian scene graph to keep track of dependencies among evaluation questions (e.g. to answer ``is the horse in air'', the question ``is there a horse'' needs to hold true first). 
This approach ensures that invalid questions do not affect the faithfulness result. 
% \maneesh{Do we use Davidsonian graphs in our work. If so we should probably describe them in more detail using a figure.}
% \maneesh{How does our work differ from these. What are the limitations of these methods?}
In our work, we account for dependencies among constraints by decomposing complex expressions into atomic predicates chained together with logical operators (Figure~\ref{fig:teaser}).


% scenecraft
SceneCraft~\cite{hu2025scenecraft} utilizes LLMs to both synthesize and verify 3D scene programs.
They use an LLM as a ``planner'' to convert input scene descriptions into a scene graph that expresses constraints between objects.
The LLM then act as a ``coder'' to produce a scene program based on the graph.
% \maneesh{Not sure what an ``LLM coder'' is. Should explain.}
Later, another LLM instance verifies if the generated program satisfies the constraints described in the scene graph as a reviewer.
If not, the reviewer asks the LLM coder to generate a revised programs for improvement.
% \maneesh{Does it ask for a ``new'' program or a ``revision''. Should state limitations and why we are better.}
%
% \maneesh{Should explain why semantic parsing is preferable to using an LLM here and in the introduction. What can we handle that previous approaches cannot handle?}
In our work, we adopt the program synthesis with verification
approach. 
However, the non-deterministic nature of LLMs and VLMs makes them less reliable as verifiers~\cite{brown2024large}.
Therefore, we build a rule-based semantic parser based on syntactic parsing, pattern matching, and text classification to convert input motion graphics prompts into a verification program written in our proposed FOL-based DSL.


%% scene language related work

% ~\cite{sueyoshi2024predicated}
% frameNet: https://framenet.icsi.berkeley.edu/

% LocalWords:  LLMs CarSim WordNet Zhang et al pre labeler ARF LLM
% LocalWords:  KeyFramer SVG LogoMotion VLM SVGs ToonCrafter VISPROG
% LocalWords:  ViperGPT neuro DSL VLMs TIFA Cho cho davidsonian Artzi
% LocalWords:  davisonian SceneCraft disjunctions Zettlemoyer CCG Hsu
% LocalWords:  shortcite Reddy binarization binarized zhang artzi
% LocalWords:  ModelScope VideoCrafter Videofusion iteratively intra
% LocalWords:  verifiers


==> table_eval_pipeline_no_mover.tex <==
\begin{table}[t]
% \small
% \footnotesize
% \scriptsize
\centering
\caption{%
\camready{%
Performance of our pipeline with the verification report replaced by \textit{``The animation program you generated does not produce the correct animation. Please correct the animation program.''}
We observe significant increases in the number of failed prompts. Note that failed prompts are excluded from the average and min-max iteration metrics.
The slight differences in pass@0 are the results of using a temperature of 1.0.
We used a seed of 1 to mitigate the inherent randomness of LLM generation.%
% \maneesh{What is this table showing? The caption is super confusing as the naming of the tables is not very clear. These should likely be two separate tables and they need to be named clearly. "Simple sampling" is not clear at all. Not clear why some of these numbers for pass@0 are different from table 3. I would assume both of these tablews to have the same numbers for pass@0 as in tbale 3. The numbers don't make any sense. These experiments need to be added carefully.}
}%
}
\vspace{-1em} %% commented out for arxiv
\resizebox{\linewidth}{!}{%
\begin{tabular}{lrrrrr}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Pipeline\\w/ coarse\\report \end{tabular}} & \multicolumn{5}{c}{Prompt Type}                     \\ \cline{2-6}
                                 & \begin{tabular}[c]{@{}c@{}}Single\\atomic\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spatially\\relative\end{tabular} & \begin{tabular}[c]{@{}c@{}}Temporally\\relative\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spatio-\\temporally\end{tabular}  & \multicolumn{1}{|c}{Overall} \\
\hline
pass@0                 & 1061 (88.4\%) & 532 (38.0\%)   & 1059 (88.3\%)  & 636 (35.3\%) & \multicolumn{1}{|r}{3288 (58.7\%)}    \\
pass@1+                & 129 (10.8\%)  & 418 (29.9\%)   & 133 (11.0\%)   & 394 (21.9\%) & \multicolumn{1}{|r}{1074 (19.2\%)}    \\
fail                   & 10 (0.8\%)    & 450 (32.1\%)   & 8 (0.7\%)      & 770 (42.8\%) & \multicolumn{1}{|r}{1238 (22.1\%)}    \\
\cline{1-6}
avg. iters.            & 2.6 (1-21)    & 3.6 (1-37)     & 1.6 (1-8)      & 6.7 (1-37)   & \multicolumn{1}{|r}{4.4 (1-37)}    \\
\bottomrule
\end{tabular}%
} % end resize
\label{tab:eval_pipeline_no_mover_coarse}
\end{table}


\begin{table}[t]
% \small
% \footnotesize
% \scriptsize
\centering
\caption{%
\camready{%
Performance of our pipeline with the verification report replaced by \textit{``Generate an animation following the same prompt.''}
Note the highest numbers of failed prompts across all prompt types.}
}
\vspace{-1em} %% commented out for arxiv
\resizebox{\linewidth}{!}{%
\begin{tabular}{lrrrrr}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Pipeline\\w/ no\\feedback\end{tabular}} & \multicolumn{5}{c}{Prompt Type}                     \\ \cline{2-6}
                                    & \begin{tabular}[c]{@{}c@{}}Single\\atomic\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spatially\\relative\end{tabular} & \begin{tabular}[c]{@{}c@{}}Temporally\\relative\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spatio-\\temporally\end{tabular}  & \multicolumn{1}{|c}{Overall} \\
\hline
pass@0                 & 1062 (88.5\%) & 528 (37.7\%)   & 1064 (88.7\%)   & 646 (35.9\%) & \multicolumn{1}{|r}{3300 (58.9\%)}    \\
pass@1+                & 43 (3.6\%)    & 314 (22.4\%)   & 118 (9.8\%)     & 200 (11.1\%) & \multicolumn{1}{|r}{675 (12.1\%)}    \\
fail                   & 96 (8.0\%)    & 558 (39.9\%)   & 18 (1.5\%)      & 954 (53.0\%) & \multicolumn{1}{|r}{1626 (29.0\%)}    \\
\cline{1-6}
avg. iters.            & 7.0 (1-32)   & 3.8 (1-35)      & 1.6 (1-10)      & 2.8 (1-38) & \multicolumn{1}{|r}{3.3 (1-38)}    \\
\bottomrule
\end{tabular}%
} % end resize
\label{tab:eval_pipeline_no_mover_another}
\end{table}
